Classifying and Propagating Parity Constraints (extended version)

Parity constraints, common in application domains such as circuit verification, bounded model checking, and logical cryptanalysis, are not necessarily most efficiently solved if translated into conjunctive normal form. Thus, specialized parity reasoning techniques have been developed in the past for propagating parity constraints. This paper studies the questions of deciding whether unit propagation or equivalence reasoning is enough to achieve full propagation in a given parity constraint set. Efficient approximating tests for answering these questions are developed. It is also shown that equivalence reasoning can be simulated by unit propagation by adding a polynomial amount of redundant parity constraints to the problem. It is proven that without using additional variables, an exponential number of new parity constraints would be needed in the worst case. The presented classification and propagation methods are evaluated experimentally.

==> treelikeproportions.tex <==
\begin{figure}
\begin{tabular}{|l|c|c|c|}
\hline
\textbf{Benchmark}
& \textbf{\# variables}
& \textbf{\# xor-clauses}
& \textbf{\# xor-clauses tree-like}
\\
\hline
DES (4 rounds 2 blocks) 
& 3781
& 320
& 192 \\

Grain (16 bit)
& 9240
& 6611
& 659 
\\

Hitag2 (33 bit) 
& 6010
& 3747
& 1018
\\

\Trivium{} (16 bit)
& 11485
& 8591
& 0
\\

Atree (40, SAT) 
& 13557
& 3158
& 3156
\\

Braun (40, SAT)
& 12061
& 1520
& 1514
\\
\hline
\end{tabular}
\caption{Number of tree-like xor-clauses on some benchmarks. The numbers represent the medians computed from the whole benchmark set (5-51 instances / benchmark)}
\label{Fig:TreeLikeProportions}
\end{figure}

